From Curves to Words and Back Again: Geometric Computation of Minimum-Area Homotopy

Let $\gamma$ be a generic closed curve in the plane. Samuel Blank, in his 1967 Ph.D. thesis, determined if $\gamma$ is self-overlapping by geometrically constructing a combinatorial word from $\gamma$. More recently, Zipei Nie, in an unpublished manuscript, computed the minimum homotopy area of $\gamma$ by constructing a combinatorial word algebraically. We provide a unified framework for working with both words and determine the settings under which Blank's word and Nie's word are equivalent. Using this equivalence, we give a new geometric proof for the correctness of Nie's algorithm. Unlike previous work, our proof is constructive which allows us to naturally compute the actual homotopy that realizes the minimum area. Furthermore, we contribute to the theory of self-overlapping curves by providing the first polynomial-time algorithm to compute a self-overlapping decomposition of any closed curve $\gamma$ with minimum area.

==> body/append-foldings.tex <==
%!TEX TS-program = pdflatex
%!TEX encoding = UTF-8 Unicode
%!TeX spellcheck = en-US
%!TeX root = ..\sosa22.tex

%-----------------------Foldings------------------------------------
\section{Omitted Proofs On Foldings}
\label{append:foldings}

In this section, we include proofs from \secref{interpretation}.
First, the proof that for each folding there is a homotopy with equal area.

\foldingarea*

\begin{proof}
	We induct on the number of pairings in $F$.
    %
    Consider a folding $F$ with $k$ pairings, and let $(\str{f},\str{\bar{f}})$ be a pairing in $F$ that does not contain any other pairing in between.
	A Blank cut along this pairing decomposes
	the curve into two subcurves, at least one of which does not
	contain any pairings. 
    Call this subcurve $\curve_1$.
	We will contract $\curve_1$ to the cut using a homotopy
	with area equal to the sum of area of all the unpaired letters in the subword of $\curve_1$; such homotopy exist by the base case of induction.
    %
	However, after we contract $\curve_1$,
	the cable system on the remaining curve might no longer be managed or shortest, and there might be multiple cables in some faces.
	Therefore we strengthen the inductive hypothesis by assuming that for any subword of $[\gamma](\Pi)$ and its corresponding subcurve $\curve'$ of $\gamma$ with the induced (unmanaged multi-)cable system, and a folding $F'$ with less $k$ pairings on the subword,
	there exists a null-homotopy of $\curve'$ with area equal to the area of the folding $F'$, and the destination of the null-homotopy can be anywhere on $\curve'$. 
	
    Let $w'$ be the subword of $[\gamma](\Pi)$ by removing the subword between the pairing $(\str{f},\str{\bar{f}})$, folding $F'$ on subword $w'$ be constructed from $F$ by removing the pairing $(\str{f},\str{\bar{f}})$.
    Let $\curve'$ denote the curve that results from contracting
	$\curve_1$ to the cut and let $\Pi'$ denote the cable system
	induced on $\curve'$ by $\Pi$.
	By the (strengthened) induction hypothesis $\curve'$ has a null-homotopy with area equal to the one of $F'$.
    Combining with the null-homotopy of $\gamma_1$ and we are done.

    For the base case when $F$ is the empty pairing, 
    if the cables are not managed, construct a managed cable system satisfying the shortest path assumption $\Pi^*$ for $\curve$ and 
    apply Lemma~\ref{lem:independence};
    the sum of weights of all letters in the new Blank word remains unchanged.
    % to ensure that the null-homotopy to be constructed can be done without loss of generality to be with respect to the managed cable system $\Pi^*$.
    %
    To construct the null-homotopy,
    decompose the curve into depth cycles by performing a smoothing at each vertex~\cite{changErickson17},
	to obtain a null-homotopy with area equal to the depth area.
	Since each cable in $\Pi^*$ follows a shortest path to the unbounded face, the number of times an unsigned letter
	appears in the word is equal to the depth of the face,
	and thus the homotopy area is equal to the area of the folding.
    In fact, we can choose any point on the curve to be the destination of the null-homotopy.
    % Let $\curve'$ denote the curve that results from contracting
	% $\curve_1$ to the cut and let $\Pi'$ denote the cable system
	% induced on $\curve'$ by $\Pi$.
    % Now Decompose $\curve_1$ into simple depth cycles.
	% Contracting the simple depth cycles to the cut
	% gives a homotopy of $\curve_1$ with area equal to the depth
	% of each face in $\curve_1$.
	% The depth of a face in $\curve$ is equal to the depth
	% of the face in $\curve_1$ plus the depth of the face
	% in $\curve \backslash \curve_1$.
	% We apply in the inductive hypothesis and this proves the lemma.
\end{proof}

% Next, we prove that every self-overlapping decomposition determines
% a folding.

%\sodtofolding*
\subsection{Proof Lemma~\ref{lem:independence}: Cable Independence}
\label{SS:independence}


What we are left with is to prove Lemma~\ref{lem:independence}:
Given a curve $\gamma$ and a cable system $\Pi$, if we have a folding on the face word $[\gamma](\Pi)$, there is an equivalent folding of the new word $[\gamma](\Pi')$ that has the same area if we choose a different cable system.
As a result, the cancellation norm and the positive foldability of a word
are independent to the cable system chosen.
%
Notice that it is sufficient to assume $\Pi'$ to be a managed cable system with shortest path assumptions and single cable to each face.

Any two cable systems can always be connected by a sequence of isotopy and  order switching between two adjacent cables, followed by a redrawing of the cables induced by a homeomorphism of the plane fixing the punctures $\set{p_i}$, which fixes the cable ordering and the disjointness between cables but the isotopy classes of the cables change.
We emphasize that either operation will change the Blank word, but we can always find a folding of the new word that preserves the area.

%\paragraph*{Switching cable orders.}

In \appendref{foldings} we show that switching two adjacent cables preserves the area and positivity of the folding.
We summarize the result in the following lemma.

\begin{restatable}[Switch Invariance]{lemma}{normswitch}
\label{lem:norm-switch}
    %
    Given curve $\curve$, a cable system $\Pi$, and a folding $F$ on $\word(\Pi)$.
    Switching the order of two adjacent cables produces another folding on the new word with equivalent area.
    Furthermore, the new folding is positive if and only if $F$ is.
    %
\end{restatable}



% As a corollary we have the following.

% \begin{corollary}[Switching Cables and Positive Foldings]
% \label{cor:order-grouping}
% Switching the order of two adjacent cables in the rotation system
% does not change if the word is positively foldable.
% \end{corollary}

% \begin{proof}
% If $w$ is foldable with positive folding $F$, then the folding $F'$ in \lemref{norm-switch}
% is a positive folding of the $w'$ after the order of two cables has been switched.
% \end{proof}


%\paragraph*{Converting between cable systems with the same ordering.}

Next, we show that the cancellation norm does not depend on the
cables having the shortest path property.
While the face word is unique up to isotopy of the cables based on \lemref{isotopy}, two cable systems with identical ordering around $p_0$ may not be isotopic to each other.
The theory of mapping class groups~\cite{primer,martelli2016}
provides tools to convert between all possible isotopy classes of cable systems with same cable ordering.

% \brittany{it seems we've transitioned into background on mapping class groups.
% Should this be in the background?}
% \brad{The mapping class group ideas are not used until here, I
% worry the reader will have forgotten about them by the time they get here}
Let \EMPH{$S_{g,n}$} denote a surface with genus $g$
and $n$ punctures.
Let \EMPH{$\text{Diffeo}^+(S_{g,n})$} denote the group of all orientation-preserving diffeomorphisms from $S_{g,n}\to S_{g,n}$.
Define an equivalence relation~$\sim$ on $\text{Diffeo}^+(S_{g,n})$, where
$\phi\sim \psi$ if there exists an isotopy between $\phi$ and $\psi$.
%
The \EMPH{mapping class group} of $S_{g,n}$ is the group
\(
\textnormal{MCG}(S_{g,n}) = \textnormal{Diffeo}^+(S_{g,n})\slash \sim.
\)
A simple closed curve or a puncture-to-puncture arc $\lambda$ on a surface is \EMPH{nonseparating} if the surface remains connected after cutting along $\lambda$.
A simple closed curve (or arc) in a surface is \EMPH{essential}
if it is not homotopic to a point and not homotopic to a puncture.

Let $\lambda$ be a simple closed curve in a surface.
We now describe a particular mapping class in $\textnormal{MCG}(S_{g,n})$, a \EMPH{Dehn twist} --- about $\lambda$.
Let $A_\lambda$ be an arbitrarily thin annulus homeomorphic to the product of $\Sp^1$ and the unit interval $I$; i.e.\ $A_\lambda \cong \Sp^1 \times I$
with $\lambda\cong \Sp^1\times \{0\}.$
The twist is the map $T_\lambda: A_\lambda \to A_\lambda$ where $T_\lambda(\theta,t)=(\theta+ 2\pi t,t)$~\cite{primer}.
Intuitively, we can think of $T_\lambda$ as acting on any path that crosses $A_\lambda$ by fixing one boundary component of the annulus
and rotating the other boundary component one full revolution, dragging all masses within $A_\lambda$ along.
See \figref{dehn-twist} for an example.
Dehn twists are well-defined as element in $\textnormal{MCG}(S_{g,n})$ and depend only on the isotopy class of $\lambda$ \cite{martelli2016}.


\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{dehn-twist/pre-dehn-twist}
        % \caption{Before the twist.}
        \label{fig:pre-twist}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{dehn-twist/post-dehn-twist}
        % \caption{After the twist.}
        \label{fig:post-twist}
    \end{subfigure}

    \caption{
        An illustration of a Dehn twist.
}
    \label{fig:dehn-twist}
\end{figure}


Let $D_n$ be the closed disk $\mathbb{D}^2$ with $n$ punctures.
The \EMPH{pure mapping class group} of $D_n$, $\textnormal{PMCG}(D_n)$,
is the subgroup of $\textnormal{MCG}(D_n)$ that fixes all punctures.
The group $\textnormal{PMCG}(D_n)$ is generated by a finite number
of closed curves.

\begin{theorem}[Generators~{\cite[\S9.3]{primer}}] \label{thm:generators}
$\textnormal{PMCG}(D_n)$ is generated by Dehn twists
about the set of simple closed curves that surround exactly two punctures.
%\hsien{Careful. Does actual drawing of the closed curves matter?}
\end{theorem}

%Each cable is an essential arc between punctures.
Thus, given any cable system we can perform Dehn twists about these generators to obtain another cable system with the same cable ordering such that all cables are shortest paths.
We choose a disk in the plane that contains the curve $\gamma$, the punctures, and the cables.
(One subtlety is that even when the two cable systems have the same \emph{cyclic} ordering, the choice of the disk may produce different \emph{linear} cable ordering when we decide the location to take the containing disk.  This can be easily resolved by redrawing some of the cables using isotopy across the infinity.)
We now show that performing Dehn twists about suitable simple closed curves does not change the cancellation norm of the word.
%\hsien{Subtlety: even with same cyclic cable ordering, the choice of the disk may give different linear cable ordering.  Urr.  Secondary.}


\begin{lemma}[Twist Invariance]\label{lem:norm-twist}
    Let $\gamma$ be a curve and $\Pi$ be a cable system, and let $F$ be a folding on the corresponding face word $[\gamma](\Pi)$.
    Dehn twists about the cables in $\Pi$ produce another folding on the new word with equal area.
\end{lemma}


\begin{proof}
Let $\Pi$ be a cable system on a closed curve $\gamma$.
Given two punctures $p_i$ and $p_j$, let $c_{i,j}$
denote the closed curve that contains only
$p_i$ and $p_j$ and follows the cables $\pi_i$ and $\pi_j$
to the exterior face, then connect.
See \figref{pre-twist} for an illustration.
There may be cables
between $\pi_i$ and $\pi_j$ in the rotation order about $p_0$.
We bundle all such cables together and denote the corresponding face word \EMPH{$B$}.
By \thmref{generators}, the closed curves $c_{i,j}$s generate the pure mapping
class group.
%
To show that twisting about $c_{i,j}$ does not change the norm,
let $w$ be the word generated by the cables before twisting about
$c_{i,j}$ and let $w'$ be the word generated by the cables after the twist.
We will show that $||w'||\leq ||w||$ and $||w||\leq ||w'||$.

Instances of $\str{f_i}$ and $\str{\bar{f}_i}$ in $w$ become
$(\str{\bar{f}_i}\bar{B}\str{\bar{f}_j}{B}) \str{f_i} (\bar{B}\str{f_j}{B}\str{f_i})$ and
$(\str{\bar{f}_i}\bar{B}\str{\bar{f}_j}{B}) \str{\bar{f}_i} (\bar{B}\str{f_j}{B}\str{f_i})$ in $w'$.
Instances of $\str{f_j}$ and $\str{\bar{f}_j}$ in $w$ become
$(B\str{\bar{f}_i}\bar{B}\str{\bar{f}_j}) \str{f_j} (\str{f_j}B\str{f_i}\bar{B})$ and
$(B\str{\bar{f}_i}\bar{B}\str{\bar{f}_j}) \str{\bar{f}_j} (\str{f_j}B\str{f_i}\bar{B})$ in $w'$.
See \figref{do-the-twist} for an example.

\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\textwidth]{twist/twist-about-gamma}
            \subcaption{Before the twist.}\label{fig:pre-twist}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\textwidth]{twist/twisted}
        \subcaption{After the twist.}\label{fig:post-twisted}
    \end{subfigure}

    \caption{
    (\subref{fig:pre-twist})
    An example of the Dehn twist.
    The curve is shown in black.
    Starting from the star and following the indicated orientation, the Blank word is $w = [\str{23142\overline{34}}]$.
    In the instance we have $i=4$ and $j=3$;
    the curve $c_{4,3}$ is shown in gray.
    The word $B$ is $\str{1}$.
    (\subref{fig:post-twisted}) After twisting about an annulus formed by fattening $c_{4,3}$ the new word is
    $w' = [\str{2}\strp{1\overline{413}}\str{3}\strp{314\overline{1}}\str{1}\strb{\overline{413}1}\str{4}\strb{\overline{1}314}\str{2}
    \strp{1\overline{413}}\str{\overline{3}}\strp{314\overline{1}}\strb{\overline{413}1}\str{\overline{4}}\strb{\overline{1}314}]$.
    }
    \label{fig:do-the-twist}
\end{figure}

We now construct a folding $F'$ of $w'$ with equal area.
All pairs in $F$ are in $F'$. All letters added by the twist are then paired.
If $\str{f_i}$ is in $w$ and unpaired in $F$ then we pair the conjugate letters
on each side of $\str{f_i}$ in $w'$.
If $\str{f_i}$ is in $w$ and paired in $F$ then
we pair the added letters to the right of $\str{f_i}$ with the added letters to the left of the paired $\str{\bar{f}_i}$ in $w'$;
similarly, we pair the added letters to the left of $\str{f_i}$ with the added letters to the right of $\str{\bar{f}_i}$.
This can be done because the added words are the same mirror pair around symbol $\str{f_i}$ and $\str{\bar{f}_i}$.
\[
w' = [\ldots (\str{\bar{f}_i}\bar{B}\str{\bar{f}_j}{B}) \overbracket{\str{f_i} (\bar{B}\str{f_j}{B}\str{f_i})
\ldots (\str{\bar{f}_i}\bar{B}\str{\bar{f}_j}{B}) \str{\bar{f}_i}} (\bar{B}\str{f_j}{B}\str{f_i}) \ldots]
\]
where the overbracket indicates the pairing $(\str{f_i},\str{\bar{f}_i})$.
Thus, a folding of $w'$ of equal area exist.  Because the cancellation norm is computed by taking minimum over all foldings, we have $||w'||\leq ||w||$.

On the other hand, given a folding $F'$ of $w'$ we construct a folding $F$ of $w$ with area at most the area of $F'$.
If an element of $w$ is unpaired in $F'$ it is also unpaired in $F$.
There are three types of pairings in $F'$.
%
If both letters in the pair are in $w$: in which case we add this pair to $F$.
%
If neither letter in the pair is in $w$, in which case we do nothing to $F$.
%
The third type of pairing contains a letter of $w$ paired with a letter
in that only presents in $w'$ but not in $w$;
call this pair $(\str{f}^0,\str{\bar{f}}^1)$ where $\str{f}^0$ is in $w$ and
$\str{\bar{f}}^1$ is in $w'\backslash w$.
We will show that there is a unique unpaired letter $\str{f}^k \in w'\backslash w$
that is left unpaired in $F$,
%contributes the area of face corresponding to $\str{f}^0$,
or there is another $\str{\bar{f}}^k\in w$
that we can pair $\str{f}^0$ with in $F$.

We construct a sequence of letters in $w'$ that are all $\str{f}$ and $\str{\bar{f}}$s and terminates with either an unpaired letter in $w'\backslash w$
or a paired letter in $w$.
%
Let $P$
%$P:\set{\text{letters}}\to \set{\text{letters}}$
denote the function
that maps a letter to its paired letter in $F'$, or the identity otherwise.
%Letters in $w'\backslash w$ come in inverse pairs as conjugates.
The map $C$
%$C:\set{\text{letters}}\to \set{\text{letters}}$
maps a letter of $w'\backslash w$ to its conjugate inverse in the mirror pair added by the Dehn twist if the conjugate inverse has not yet been visited, or the identity otherwise.
Note that both $P$ and $C$ are injective, and they only map a symbol $\str{f}$ to its inverse $\str{\bar{f}}$ and vice versa.
%
Beginning with the pairing $(\str{f}^0,\str{\bar{f}}^1)$, we alternate in applying the functions $P$ and $C$: for any integer $i$, let
$\str{f}^{2i} \coloneqq C(\str{f}^{2i-1})$ and
$\str{f}^{2i+1} \coloneqq P(\str{f}^{2i})$.
% \[
% \begin{aligned}
% \str{f}^{2i} \coloneqq C(\str{f}^{2i-1}), \\
% \str{f}^{2i+1} \coloneqq P(\str{f}^{2i}).
% \end{aligned}
% \]
Since the word is finite, this unique sequence terminates with
either an unpaired letter $\str{f}^k$ of $w'\backslash w$
%with weight equal to $\str{f}^0$
or an element $\str{\bar{f}}^k$ in $w$.

\begin{itemize}\itemsep=0pt
\item
If the sequence of letters ends with an unpaired letter in $w'\backslash w$,
this letter uniquely corresponds to $\str{f}^0$ by following pairings
and corresponding inverses in $F'$.
%
For example,
let $F'$ be the folding indicated by the overbrackets,
with the underbrackets denoting corresponding conjugate inverse~letters,
\[
[\str{2}\strp{1\overline{413}}
\rlap{$\overbracket{\phantom{\str{3}\strp{314\overline{1}}\str{1}\strb{\overline{41}}\strb{\overline{3}}}}$}
\str{3}\strp{314\overline{1}}\str{1}\strb{\overline{41}}
\rlap{$\underbracket{\phantom{\strb{\overline{3}} \strb{1}\str{4}\strb{\overline{1}} \strb{3}}}$}
\strb{\overline{3}} \strb{1}\str{4}\strb{\overline{1}}
\rlap{$\overbracket{\phantom{\strb{314}\str{2}\strp{1\overline{41}} \strp{\overline{3}}}}$}
\strb{314}\str{2}\strp{1\overline{41}}
\rlap{$\underbracket{\phantom{\strp{\overline{3}}\str{\overline{3}}\strp{3}}}$}
\strp{\overline{3}}\str{\overline{3}}\strp{3}
\strp{14\overline{1}}\strb{\overline{413}1}\str{\overline{4}}\strb{\overline{1}314}].
\]
The unique unpaired letter corresponding to $\str{3}$ is $\strp{3}$
found by considering the second corresponding inverse letter.

\item
If the sequence of letters ends with a letter $\str{f}^k$ in $w$,
we pair $\str{f}^0$ and $\str{\bar{f}}^k$ in $F$.
This does not create any linked pairs in $F$ since
$\str{f}^0$ and $\str{\bar{f}}^k$ participate in pairings in $F'$,
they are not linked by any other pairing in $F'$.
%
For example,
let $F'$ be the folding indicated by the overbrackets,
with the underbrackets denoting corresponding conjugate inverse letters,
\[
[\str{2}\strp{1\overline{413}}
\rlap{$\overbracket{\phantom{\str{3}\strp{314\overline{1}}\str{1}\strb{\overline{41}}\strb{\overline{3}}}}$}
\str{3}\strp{314\overline{1}}\str{1}\strb{\overline{41}}
\rlap{$\underbracket{\phantom{\strb{\overline{3}} \strb{1}\str{4}\strb{\overline{1}} \strb{3}}}$}
\strb{\overline{3}} \strb{1}\str{4}\strb{\overline{1}}
\rlap{$\overbracket{\phantom{\strb{314}\str{2}\strp{1\overline{413}} \str{\overline{3}}}}$}
\strb{314}\str{2}\strp{1\overline{413}}\str{\overline{3}}\strp{3}
\strp{14\overline{1}}\strb{\overline{413}1}\str{\overline{4}}\strb{\overline{1}314}].
\]
The pairing $(\str{3,\overline{3}})$ is then added to $F$.
\end{itemize}

\noindent The sum of the areas of the unpaired letters of $F$ is at most the sum
of the areas of the unpaired letters of $F'$ and thus $||w||\leq ||w'||$.
This proves the lemma.
\end{proof}


We show the invariance for positive foldability in \appendref{foldings}.

\begin{restatable}
%[Positive fodability is Cable Invariant]
{lemma}{groupabletwist}
%\begin{lemma}[Positive fodability is Cable Invariant]
\label{lem:groupable-twist}
Being positively foldable does not depend on Dehn twists.
\end{restatable}


Together, \lemref{norm-switch} and \lemref{norm-twist} imply the cancellation
norm does not depend on the isotopy class of the cables. Moreover,
\lemref{norm-switch} and \lemref{groupable-twist} imply the positive foldability of the word does not depend on the isotopy class of the cables.
One last subtlety: we show that we can handle multiple cables
per face in \appendref{foldings}.
This proves Lemma~\ref{lem:independence}.


Next, we include the proof that the cancellation norm is invariant 
under switching the order of the cables.

\normswitch*

\begin{proof}
Consider two cables $\pi_f$ and $\pi_g$ in $\Pi$ that are adjacent in the rotation system.
Assume $\pi_g$ is in the clockwise direction of $\pi_f$
in the rotation system and we are trying to move $\pi_f$ across $\pi_g$.
Let $w \coloneqq [\curve]_B(\Pi)$ denote the Blank word before the order of the cables are switched and $w'$ the word after the cables are switched; by Lemma~\ref{lem:isotopy} the words are well-defined up to isotopy classes of $\pi_f$ and $\pi_g$.
%
First, we argue that, without loss of generality, we can assume the drawing of $\pi_g$ follows $\pi_f$ in an $\e$-neighborhood before continuing towards puncture $p_g$, by drawing $\pi_g$ still counter-clockwise to and $\e$-close to $\pi_f$ from $p_0$ to $p_f$ and back to $p_0$, followed by the original drawing of $\pi_g$.  
The new drawing is disjoint from the rest of the cables and is isotopic to the original drawing.
This way we can ensure any instance of symbol $\str{f}$ in $w$ is followed immediately by a $\str{g}$, and
any instance of $\str{\bar{f}}$ has a $\str{\bar{g}}$ proceeding in the word.
(Notice we cannot necessarily say the same about $\str{g}$ because cable $\pi_g$ continues after reaching $p_f$.)

% Perform an isotopy so that $\pi_g$ follows beside $\pi_f$ from the puncture $p_f$ to the exterior face.
% Any instance of $\str{f}$ in $W$ has $\str{g}$ following in the word, and
% any instance of $\str{\bar{f}}$ has $\str{\bar{g}}$ proceeding in the word.

Let $F$ be a folding of $w$, we construct a folding $F'$ of $w'$
with equal area.  We separate into two cases.
%
If no instance of $(\str{f},\str{\bar{f}})$ is in $F$, then all pairings in $F$ can be paired in $W'$ and we can set $F' \coloneqq F$.
%
Now we assume there is an instance of $(\str{f},\str{\bar{f}})$ in $F$.
We further split into subcases.
Look at the two $\str{g}$/$\str{\bar{g}}$ symbols adjacent to the $(\str{f},\str{\bar{f}})$ pair in $F$.
%
If the two $\str{g}$ symbols is a pairing in $F$, then we can again set $F' \coloneqq F$.
If exactly one of the $\str{g}$/$\str{\bar{g}}$ adjacent to the $(\str{f},\str{\bar{f}})$ pair is the paired with another $\str{\bar{g}}$ or $\str{g}$ that is not adjacent to the $(\str{f},\str{\bar{f}})$ pair in $w$,
then switching the cables na\"ively results in a linked pair,
    \[
    w = [\ldots \underbracket{\str{f} \str{g} \ldots \overbracket{\str{g} \ldots \str{\bar{g}}}\str{\bar{f}}}\ldots] 
    \longrightarrow  
    w' = [\ldots\str{g} \rlap{$\underbracket{\phantom{\str{f}\ldots \str{g} \ldots \str{\bar{f}}}}$}\str{f}\ldots
    \overbracket{\str{g} \ldots \str{\bar{f}}\str{\bar{g}}}\ldots].
    \]
Instead, after the cables are switched, we pair the $\str{g}$ and $\str{\bar{g}}$ that appear next to the $(\str{f},\str{\bar{f}})$ pair together in $F'$:
\[
    w' = [\ldots  \underbracket{\str{g} \overbracket{\str{f} \ldots \str{g} \ldots \str{\bar{f}}} \str{\bar{g}}}\ldots].
\]
The new $F'$ is a folding without linked pairs and does not change the area because the same number and types of symbols are paired.
%
Finally, if both $\str{g}$ and $\str{\bar{g}}$ adjacent to the $(\str{f},\str{\bar{f}})$ pair are paired with letters not adjacent to $\str{\bar{f}}$ and $\str{f}$ in $F$,
we pair $\str{g}$ next to the $\str{f}$ with the $\str{\bar{g}}$ next to $\str{\bar{f}}$ and the $\str{g}$ not adjacent to the $\str{f}$ with the $\str{\bar{g}}$
not adjacent to $\str{\bar{f}}$ in $F'$:
   \[
   w = [\ldots \underbracket{\str{f} \overbracket{\str{g} \ldots \str{\bar{g}}}\ldots \overbracket{\str{g} \ldots \str{\bar{g}}}\str{\bar{f}}}\ldots] 
   \longrightarrow
   w' = [\ldots \underbracket{\str{g} \overbracket{\str{f} \ldots \underbracket{\str{\bar{g}}\ldots \str{g}} \ldots \str{\bar{f}}}\str{\bar{g}}}\ldots].
   \]
Again, $F'$ remains a folding without linked pairs and has the same area as $F$. 
\end{proof}

\paragraph*{Handling multiple cables per face.}


When a face $f$ in a subcurve contains multiple cables and punctures, we treat the punctures as distinct when applying \lemref{norm-switch} and \lemref{norm-twist}.
Now, once all the cables follow the cotree shortest paths, consider all cables ending in an arbitrary face $f$.
If they are separated by other cables in the cyclic ordering, we use \lemref{norm-switch} and isotopy to move all the cables not ending in $f$ out of the way until they no longer intersect the face. 
This makes sure that all the cables ending in $f$ are gathered together in the cyclic ordering.
Because they follow the same unique cotree path to the exterior, we can merge them into a single cable, where the corresponding symbols in the word are merged into a single symbol with the combined weight.
Thus, the subwords induced by a face pairing correspond to the subcurves generated by the Blank cut.

\paragraph*{Min-Area Self-Overlapping Decomposition in Polynomial Time}
Finally, we show how to construct a self-overlapping decomposition 
from a maximal folding with equal area.
Before we begin the proof, we include definitions that
will help describe the types of curves we encounter.
%
A curve $\curve$ is a \EMPH{$k$-stack} if it has rotation number $k$, all bounded faces have positive winding numbers, and 
$\Area_H(\gamma)=\Area_W(\gamma)$ (see \figref{2stack} for any example).
Any $k$-stack has a vertex decomposition into $k$ self-overlapping curves~\cite[Theorem~2.15]{evans18}.%
\footnote{$k$-stacks are called \EMPH{interior-boundaries} by Titus~\cite{titus} and the terminology was used in various previous work~\cite{marx74,fkw2017,evans18}.  The name \emph{$k$-stack} is well-justified as such curve is the boundary of a stack of $k$ disks~\cite{evans18}.}
%
A curve is a \emph{$-k$-stack} if its reversal is a $+k$-stack.
We called a curve $\gamma$ a \EMPH{stack} if $\gamma$ is a $\pm k$-stack.
%
A curve is \EMPH{good}~\cite{evans18}
if the depth of each face is equal to the absolute value of the winding number; any good curve must have $\Area_D(\gamma)=\Area_H(\gamma)=\Area_W(\gamma)$ by Equation~\ref{eq:sandwich}.  
%
Good curves are almost stacks, except that some faces might not have positive winding numbers.
A vertex of $\gamma$ is \EMPH{sign-changing} if the four incident faces have winding numbers $[1,0,-1,0]$ in cyclic order (see \figref{sign-change} for
an example).
If we smooth a sign-changing vertex of a good curve, the two induced subcurves remain good. 
We can always decompose a good curve into a collection of stacks at all the sign-changing vertices~\cite[Theorem~5.7]{evans18}.
%A \EMPH{block} of a curve is maximally connected subgraph that can not be separated at a sign changing vertex.


\begin{figure}[htb]
        \centering
        \begin{subfigure}[b]{0.3\textwidth}
      		  \includegraphics[width=\textwidth]{twist/k-stack}
		   \subcaption{A $2$-stack.}\label{fig:2stack}
        \end{subfigure}
          \hspace{.5cm}
         \begin{subfigure}[b]{0.3\textwidth}
     		   \includegraphics[width=\textwidth]{twist/sign-change-vertex}
    		    \subcaption{Sign-changing vertex.}\label{fig:sign-change}
        \end{subfigure}

		\caption{(\subref{fig:2stack}) A $k$-stack where $k=2$. Smoothing at any of the three vertices gives a self-overlapping decomposition.
		(\subref{fig:sign-change}) The vertex $v$ is a sign-changing vertex.
		\label{fig:stack}}
\end{figure}


With these definitions in hand, we now show how to construct a self-overlapping decomposition from a maximal folding with equal area.

\foldingtosod*

\begin{proof}
%Recall that a self-overlapping decomposition is a collection of vertices of $\gamma$ that are smoothed so that each induced subcurve is self-overlapping.
%Given a folding we construct a self-overlapping decomposition with the desired area.
%
Let $F$ be any maximal folding of $\word(\Pi)$.
Without loss of generality we can assume that the cable system does not cut through the interior of any face by rerouting the cables similar to Section~\ref{SS:norm}.  
By Lemma~\ref{lem:isotopy} the Blank word remains unchanged.
%\hsien{Wait.  The word changes though.}

Let $\good$ be an arbitrary subcurve generated after Blank cutting along the pairings in $F$.
The curve $\good$ is must be good: otherwise, there is a face with winding number not equal to its depth, and thus $\good$ would cross the corresponding cable from left to right and from right to left.
Therefore, we can introduce an extra pair into the folding and $F$ remains unlinked; thus $F$ would not be maximal.
%
Decomposing at all the sign-changing vertices~\cite[Theorem~5.7]{evans18} turns $\good$ into a collection of stacks, each of which can be further decomposed into collection of self-overlapping curves~\cite[Theorem~2.15]{evans18}.
% In a good curve, the only face with winding number zero is the unbounded face.
% The difference between the winding number of adjacent faces is $\pm1.$
% If a good curve has faces with both
% positive and negative winding number, the positive
% and negative faces are separated by a sign changing vertex.
% Thus, $\good$ can be decomposed at vertices into blocks with
% consistent winding number.
% See \figref{combined-word} for an example.
% \hsien{The cables in the figure is not managed.}



% \hsien{This is reproving \cite{evans18}.}
% If there were a cycle in the blocks, we would have a face with
% winding number less than the depth and the curve would not be good.
% Thus, the collection of blocks in $\good$ forms a tree.
% Since the blocks form a tree, the sign changing vertices separating the blocks
% are not linked in the combined word.
% We select these vertices include in our self-overlapping decomposition.
% This further decomposes the good subcurves into good $k$-stacks of disks.
%
% Since the $k$-stacks of disks are also good,
% each $k$-stack can be decomposed
% into $k$ simple cycles \cite{evans18}.
% Consider the combined word of any good $k$-stack of disks.
% Since the subword has finite length,
% there is a pair of vertices such that one of the subwords between
% repeated vertices does not contain another pair of vertices.
% Pairing at this vertex results in one (or both) of the subcurves
% being a simple cycle with Whitney index equal to one.
% We select this vertex for our self-overlapping decomposition.
% This decreases the rotation number of the $k$-stack of disks by one.
% We continue removing simple cycles until all subcurves have rotation
% number equal to one.
% The collect of vertices resulting from the above process
% gives a self-overlapping decomposition of the curve.

The area of the folding $F$ is equal to the number of unpaired faces in $\word(\Pi)$,
which is also equal to the sum of depth area of each good subcurve.
%
Since each subcurve $\good$ of folding is good, the depth area of $\good$ is equal to its winding area.  
Any additional decomposition of $\good$ into self-overlapping curves respects the additivity of winding areas.
%
Thus, the area of folding $F$ is equal to the area induced by our chosen self-overlapping decomposition.
\end{proof}


\groupabletwist*

\begin{proof}
Let $w$ be a word and let $w'$ be the word after a Dehn twist about
the simple closed curve $c_{i,j}$ as in the proof of \lemref{norm-twist}.
Suppose $w$ is positively foldable with folding $F$. 
Then, the folding $F'$
described in \lemref{norm-twist} is a positive folding of $w'$.

On the other hand, suppose $w'$ has a positive folding $F'$.
Then, each element $\str{\bar{f}}$ of $w'$ is paired with an element $\str{f}$.
If both $\str{\bar{f}}$ and $\str{f}$ are in $w$ then we pair them.
If neither $\str{\bar{f}}$ nor $\str{f}$ are in $w$ then we ignore them.
If one of $\str{\bar{f}}$ and $\str{f}$ are in $w$ and the other is added to $w'$ by the twist,
then, since letters are added to $w'$ in pairs, there is another element of $w$ paired
with an element of $w'\backslash w$. We can pair the two element in $w$
and ignore the two in $w'\backslash w$ because the pairings in $F'$ are not linked.
The resulting pairings give a positive folding of $w$.
\end{proof}

%Finally, we prove that every self-overlapping decomposition (with respect to the vertex word of $\gamma$) 
%determines a folding (of the face word of $\gamma$) using the combined word.

%\sodtofolding*



==> body/append-words.tex <==
%!TEX TS-program = pdflatex
%!TEX encoding = UTF-8 Unicode
%!TeX spellcheck = en-US
%!TeX root = ..\swat22.tex

%----------------------- words -------------------------------------
\section{Additional Details On Words}
\label{append:words}


In this section, 
we give a complete description of Nie's word construction
and we prove that Nie's word and Blank's word are equivalent.
First, we show  that the Blank word is unique.

\blankunique*
\begin{proof}

    We will argue that once the basepoint $p_0$ and the order of cables in $\Pi$ around $p_0$ is
    fixed, all the drawings of $\Pi$ respecting the cable ordering lead to the same Blank word.
    %
    %Consider the (planar) dual graph of $\gamma$; the cables can be viewed as a collection
    %of simple paths in the dual.
    Because the cable system is managed, the tree-cotree pair of $\gamma$ are fixed and
    we can safely contract the primal tree and treat the
    graph as a collection of nested loops.
    If the path passes through a vertex of $\gamma$, it counts as two crossings.
    We prove that all the cables to the loops at certain depth have a fixed ordering by
    induction on the depth.
    This is sufficient as any two cable systems with the same cables and ordering on every
    loop of the same depth must be isotopic, thus by \lemref{isotopy} their Blank words are identical.
    %
    Because of the shortest path assumption, there is only one way to draw the cables to the depth-1 contours.
    % Now if we denote the cable ordering of $\Pi$ as a cyclic permutation $\pi$, the cables
    %connecting to depth-1 faces partitions the rest of the symbols in $\pi$ (excluding those associated
    %with depth-1 faces) into a sequence of subwords $\pi_1, \dots, \pi_{k}$, where $k$ is the
    %number of depth-$1$ faces.
    % (Notice that some $\pi_i$ might be empty, and each $\pi_i$ is no longer cyclic.)
    % Imagine we extend the cables to the boundary of the depth-2 contours in a pairwise disjoint fashion; the cable orders on the depth-2 contours are uniquely determined.

    For any $\ell$, imagine all cables of depth at least $\ell$ are currently drawn from $p_0$
    to the depth-$\ell$ loops, where on each loop the collection of the cables are precisely
    those faced contained within the loop, and the cable ordering on the loops is fixed.
    Due to the shortest path assumption, every cable of depth $\ell$ has to terminate at their
    corresponding face.
    %
    There is at most one unique way to extend each cable of depth $\ell$ to its representative
    point in the face while keeping all depth-$\ell$ cables disjoint and simple, up to isotopy of the cables.
    (If no such drawing exist, this particular cable ordering is not realizable as a cable system.) %\note{requires a proof}
    By \lemref{isotopy}, isotopy does not change the order the curve $\gamma$
    passing through these depth-$\ell$ cables.
    %
    Now we partition the cables to faces of depth greater than $\ell$ based on
    children loops that contains the corresponding faces.
    There is one unique way to extend each cable of depth greater than $\ell$ to the
    depth-$(\ell+1)$ loops up to isotopy.
    Again by \lemref{isotopy}, isotopy does not change the order the curve
    $\gamma$ passing through the cables of depth more than $\ell$.
    %
    By induction, the Blank word of $\gamma$ is unique.
\end{proof}
\begin{figure}[htb]
    \centering
    \includegraphics[width=.3\textwidth]{mgmt/no-mgmt}
    \caption{An example of a cable system with a cable, in red, that cannot be managed.}
    \label{fig:no-mgmt}
\end{figure}

\begin{figure}[h!]
    \captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[t]{0.35\textwidth}
        \includegraphics[width=\textwidth]{blank-example/blank-word3}
        %\caption{A shortest path cable system.}
        \subcaption{}\label{fig:blank3}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}[t]{0.35\textwidth}
        \includegraphics[width=\textwidth]{blank-example/blank-word4}
        %\caption{A non shortest path cable system.}
        \subcaption{}\label{fig:blank4}
    \end{subfigure}
    %
    \caption{
        (\subref{fig:blank3}) A curve with labeled faces and edges. A shortest path cable system $\Pi_a$ is drawn in blue.
        From the indicated start position, the Blank Word is $[\gamma]_B(\Pi_a) = [\str{43254\overline{3}1}]$.
        (\subref{fig:blank4}) The same curve with a cable system $\Pi_b$ that does not fulfill the shortest path assumption. The Blank word is $[\gamma]_B(\Pi_b) = [\str{43254\overline{2}\overline{3}21}]$.
        }
        \label{fig:blank-word-bfs}
\end{figure}


\subsection{The Nie Word Construction}
\label{SS:Nie}

In an unpublished manuscript~\cite{nie2014,nie-emails}, Nie described how to
compute the minimum homotopy area between any two planar closed curves using the
language of geometric group theory.
Nie constructed a combinatorial word representing the planar closed curve,
followed by performing dynamic programming on the word based on a structure
called ``foldings'' (see Section~\ref{SS:norm}).
But first, let us describe the word construction.

Choose a point $p_i$ for each bounded face $f_i$ of $\curve$; denote the collection of points
%$\bigcup_i\set{p_i}$ 
as~\EMPH{$P$}.
Consider the punctured plane $X \coloneqq \RR^2 \setminus P$ and its fundamental group $\pi_1(X)$.
% Any closed curve $\gamma$ can be viewed as an element in $\pi_1(X)$, where all the curves homotopic to $\gamma$ is identified with $\gamma$ \note{do we want this?}.
Choose a set of generators $\Sigma$ for $\pi_1(X)$, where each $x_i$ in $\Sigma$ represents the
generator of $\pi_1(\RR^2\setminus \set{p_i}) \cong \ZZ$.

Now the fundamental group $\pi_1(X)$ is a free group over such generators, and
the curve $\gamma$ can be represented as a word over generators of $\pi_1(X)$.
However, there is more than one way to map each generator of
$\pi_1(\RR^2\setminus \set{p_i})$ into $\pi_1(X)$, due to the fact that in order
for $\pi_1(X)$ to be a group, one has to choose an endpoint $x_0$ and turn each
closed curve in $\pi_1(X)$ into a closed path connecting to $x_0$.
Nie never specified the choice of the connecting path because his algebraic formulation always gives the same answer
under any mapping of the generators.
%\hsien{Is this cable independence?  Check Nie's again.}

Nie's construction can also be interpreted combinatorially~\cite{nie-emails}.
Again consider the curve~$\curve$ as a four-regular plane graph.
Pick a tree-cotree pair $(T,T^*)$ of $\curve$ such that $T^*$ is a BFS-tree; naturally
 the tree $T$ is contractible.
For the sake of illustration, contract~$T$ into a single point~$t$; now each cotree edges is a
single closed path at $t$, enclosing at least one point in~$P$.
For our purpose of proving word equivalence, there are two natural sets of
generators for~$X \coloneqq \RR^2 \setminus P$:
%
\begin{itemize}\itemsep=0pt
    \item set of all cotree edges, and
    \item set of all face boundaries; i.e.\ sequences of cotree edges around each face containing $p_i$.
\end{itemize}
%
We now describe the change-of-basis between the two sets of generators in graph-theoretic terms.
%
Traverse $\curve$ from some arbitrary starting point and orient each edge of~$\curve$ accordingly.
Now, for each face $f_i$, define the \EMPH{boundary operator $\bdry$} by mapping face $f_i$ to the
signed cyclic sequence of edges around face $f_i$, where each edge is signed positively if it is
oriented counter-clockwise and negatively otherwise.

Now, write the curve $\gamma$ as a cyclic word over the cotree edges $T^*$ by traversing $\gamma$,
ignoring all tree edges in $T$.
We perform the following procedure inductively on the cotree $T^*$ to construct another cyclic word,
 this time as an element in the free group over the faces of~$\gamma$.
Starting from the leaves $f$ of $T^*$, rewrite each edge~$e$ bounding the face $f$ (that is, the
 dual of the unique edge connecting $f$ to its parent in~$T^*$) as a singleton word based on the
 index of $f$, with
 positive sign if edge $e$ is oriented counter-clockwise, or with negative sign otherwise.
%
Next, for any internal node $f$ of $T^*$, the boundary $\bdry f$ consists of a sequence of
(1) tree edges, (2) cotree edges to children of $f$ in $T^*$ denoted as $e_{1}, e_{2}, \ldots, e_{r}$,
and (3) (a unique) cotree edge to parent of $f$ denoted as $e_f$:
\[
    \bdry f = [e_f e_{1} e_{2} \ldots e_{r}].  %= [e_{j+1} \ldots e_{r} e_f e_{1} \ldots e_{j}].
\]
We can now inductively rewrite each child cotree edge $e_i$ as a free word $w_i$ over the faces
(and ignore all tree edges).
We emphasize that each word for the child cotree edge constructed inductively is a free word,
not a cyclic word.
Choose a particular but arbitrary way to break the cyclic sequence of faces and rewrite the equation:
\[
    e_f =  \bar{w}_{r} \cdot \cdots \cdot \bar{w}_{j+1} \cdot (\bar{w}_j)' \cdot \bdry f \cdot (\bar{w}_j)'' \cdot \bar{w}_{j-1}
     \cdot \cdots \cdot \bar{w}_1,
\]
where $\bar{w}_j = (\bar{w}_j)' (\bar{w}_j)''$ is a particular way of breaking the face word $\bar{w}_j$ into two.
%\note{Well, in fact $\bdry f$ might show up in the middle of a bundle of some children $e_i$. Rewrite.}
%
This gives us a free word over the faces for edge $e_f$, and thus by induction we have rewritten
$\gamma$ as a free word over the faces.
%\note{Blank word is cyclic?}
Finally, we can turn the free word back into a cyclic word, by observing that the cyclic permutation
of the constructed free word over the faces does not affect the element we are getting in
$\pi_1(X)$ (but as a side
 effect of choosing the basepoint $p_0$ of $\gamma$).


We call the resulting signed sequence of faces the \EMPH{Nie word} and denoted
as~$[\gamma]_N(\Sigma)$, where~$\Sigma$ is the choices we made when breaking up the
cyclic word at each cotree edge, referred to as a \EMPH{cycle flattening}.
Notice that the definition of $[\gamma]_N$ depends on how we choose to break the cyclic
edge sequences, and thus is not well-defined without specifying the choices.



% -------------------------------------------------------------------------------
\subsection{Word Equivalence}

Now we are ready to prove that the two words, one defined geometrically and the
other algebraically, are in fact equivalent.

\begin{theorem}[Word Equivalence]
    \label{lem:nie-cables}
    Let $\gamma$ be any plane curve.
    For a Nie word $[\gamma]_N(\Sigma)$ with a fixed cycle flattening~$\Sigma$, there is a
    managed cable system $\Pi$ such that the Blank word $[\gamma]_B(\Pi)$ is equal to $[\gamma]_N(\Sigma)$.
    Conversely, any managed cable system~$\Pi$ induces a cycle flattening $\Sigma$ such
    that $[\gamma]_B(\Pi)$ and $[\gamma]_N(\Sigma)$ are equal.
\end{theorem}

\begin{proof}
    First, fix a tree-cotree pair $(T,T^*)$ for $\gamma$ such that $T^*$ is a BFS-tree.
    Orient the edges of the cotree $T^*$ so that it is rooted at some fixed basepoint $p_0$.
    We prove the following statement by induction on the nodes of $T^*$ from leaves to the root,
    which implies the theorem:
    %
    \begin{quote}
        The Blank subword corresponding to any cotree edge $e$ is the same as the Nie subword
        corresponding to $e$.
    \end{quote}

    To prove the statement, we will construct the cables in $\Pi$ gradually from
    each face to~$p_0$,
    at each step stopping at the cotree edge $e$ in $T^*$.
    Let $f$ be an arbitrary non-root node in~$T^*$, and edge $e$ be the unique edge from $f$ to its
    parent in~$T^*$.
    If $f$ is a leaf, $e$ is the only edge in $\bdry f$ that is not in tree $T$.
    This means, when we write $\bdry f$ using edges not in~$T$, we have~$\bdry f = \pm e$, with
    positive sign if $e$ is oriented counter-clockwise and negative sign otherwise.
    We draw the cable from the representative point in face $f$ to $e$; there is only one possible
    way to draw the cable up to isotopy.

    If $f$ is not a leaf, let $e_1, \dots, e_r$ be other non-tree edges on $\bdry f$ besides $e$ in
    counter-clockwise order around $\bdry f$, \emph{flipping their orientation defined by traversing $\gamma$ if necessary}.
    By induction hypothesis, the Blank subword of $e_i$ is the same as its Nie subword;
    denote the Blank (or Nie) subword of $e_i$ as $w_i$.
    %
    This suggests that as we traverse $e_i$, the cables in $\Pi$ seem is exactly equal to $w_i$.
    Now we need to draw the cable $\pi_f$ from the representative point of $f$ to edge $e$.
    By construction of the Nie subword and the given cycle flattening $\Sigma$, the Blank subword
    on~$e$ must be of the form
    \[
        \bar{w}_{r} \cdot \cdots \cdot \bar{w}_{j+1} \cdot (\bar{w}_j)' \cdot f \cdot
        (\bar{w}_j)'' \cdot \bar{w}_{j-1} \cdot \cdots \cdot \bar{w}_1,
    \]
    where $\bar{w}_j = (\bar{w}_j)' (\bar{w}_j)''$ is a particular way of breaking the face word
    $\bar{w}_j$ into two. (See Figure~\ref{fig:induction}.)
    Because of the shortest path assumption, the collection of symbols inside
    each~$w_i$
    corresponds to exactly the faces contained within the region formed by
    cotree edge~$e_i$
    and the primal tree $T$.
    Thus, we extend all the cables intersecting the edges $e_1, \dots, e_r$
    to $e$, and create the representative point of face $f$ within the subregion of $f$ bounded
    by the last cable in $\bar{w}_{r} \cdot \cdots \cdot \bar{w}_{j+1} \cdot (\bar{w}_j)'$ and the first
    cable in $(\bar{w}_j)'' \cdot \bar{w}_{j-1} \cdot \cdots \cdot \bar{w}_1$.
    This way we can draw the cable $\pi_f$ so that the corresponding Blank subword is equal to
    the Nie subword.
    By induction, we have $[\gamma]_B(\Pi) = [\gamma]_N(\Sigma)$ for the constructed cable
    system~$\Pi$, which is managed and satisfies the shortest path assumption by the choice
    of $T^*$ being a BFS-tree.

    From the above construction we can recover a cycle flattening from a given managed
    cable system satisfying the shortest path property, thus the converse holds as well.
    %\note{The converse.  Need to show that any position of the representative point in $f$ gives a cycle flattening.}
\end{proof}

\begin{figure}[h!]
    \centering
    \includegraphics[width=.35\textwidth]{induction/induction}
    \caption{
        As we traverse the red edge $\gamma_r$ intersects $\str{3},\str{2}$, then $\str{1}$---the cable
        corresponding to $f_1$---then $\str{4}$.
        As we traverse the boundary of $f_1$ we traverse the red edge, followed by $\str{\overline{4}}$ and
        $\str{\overline{23}}$.
        This choice of cable system $\Pi$ corresponds to cycle flattening at $f_1$ as
        $\str{\overline{23}3214\overline{4}}$ by writing $f_1 = \overline{e_2} e_3 e_1 e_4$,
        or equivalently,  $\str{\overline{23}3214\overline{4}}=\overline{e_2} e_3 e_1 e_4$.
        The Blank subword on $\gamma_r$, with respect to the cycle flattening, is
        $e_1=\str{\overline{\overline{3}}}\str{2}\cdot\str{\overline{23}3214\overline{4}}\cdot\str{\overline{\overline{4}}}
        = \str{3214}$, as expected.
        }
        \label{fig:induction}
\end{figure}


% \begin{corollary}[Word Correspondence]\label{C:equivalence}
%     For any planar curve $\gamma$, there exists a managed cable system $\Pi$ and cycle flattening
%     $\Sigma$ such that there is a one-to-one correspondence between
%     the Blank word $[\gamma]_B(\Pi)$ and the Nie word $[\gamma]_N(\Sigma)$.
%     \todo{BTF/CW: isn't this the same as the theorem above?}
% \end{corollary}


\figref{order} gives an example demonstrating the one-to-one correspondence, for four different cable systems and cycle flattenings, on the same curve and
tree-cotree pair.
%
One consequence coming from the equivalence between two words and Lemma~\ref{lem:blank-unique}
%and the uniqueness of Blank word after fixing the cable ordering,
is that Nie word is uniquely determined after knowing
the subwords corresponding to cotree edges incident to the unbounded face.
This is not obviously from the definition of Nie word itself.

With this equivalence in hand, for the remainder of
the paper we refer to a Nie word or a Blank word of a curve $\gamma$ as the \EMPH{word}, denoted as $\word$ by dropping the subscripts.
Keep in mind, however, that the formal equivalence holds only when
the cable system is~managed.

\begin{figure}[h!]
    \captionsetup[subfigure]{justification=centering}
    \centering

    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{order/order-base}
       \subcaption{}\label{fig:order-base}
    \end{subfigure}
    \hspace{.5cm}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{order/order-trees}
        \subcaption{}\label{fig:order-trees}
    \end{subfigure}
    \hspace{.5cm}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{order/order-labels}
        \subcaption{}\label{fig:order-labels}
    \end{subfigure}\\

    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{order/order-blank-1}
        \subcaption{}\label{fig:order-blank-1}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{order/order-blank-2}
        \subcaption{}\label{fig:order-blank-2}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{order/order-blank-3}
        \subcaption{}\label{fig:order-blank-3}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{order/order-blank-4}
        \subcaption{}\label{fig:order-blank-4}
    \end{subfigure}

    \caption{
        (\subref{fig:order-base}) A curve $\gamma$.
        (\subref{fig:order-trees}) A spanning tree in red and cotree in blue.
        (\subref{fig:order-labels}) A labeling of the coedges and faces.
        We have four ways to break the cyclic face sequence for $e_1$, represented using the cable system $\Pi$:
        (\subref{fig:order-blank-1})~$e_1=\partial{f_1}e_2\overline{e_3}\overline{e_4}$;
        (\subref{fig:order-blank-2})~$e_1=e_2\partial{f_1}\overline{e_3}\overline{e_4}$;
        (\subref{fig:order-blank-3})~$e_1=e_2\overline{e_3}\partial{f_1}\overline{e_4}$; and
        (\subref{fig:order-blank-4})~$e_1=e_2\overline{e_3}\overline{e_4}\partial{f_1}$.
        }
        \label{fig:order}
\end{figure}












==> body/discussion.tex <==
%!TEX TS-program = pdflatex
%!TEX encoding = UTF-8 Unicode
%!TeX spellcheck = en-US
%!TeX root = ..\socg23.tex

%----------------------- Discussion-------------------------------------
\section{Discussion}
\label{sec:discussion}


In this work, we showed a duality between the algorithms of Blank and Nie.
Manipulating the letters of a word correspond to discrete
homotopies of the curve in a natural way.
We hope this correspondence will
be useful in other problems such as efficiently computing
homotopy height or homotopy width. See \cite{no-magic-leash,cdMo17} for a
precise statement of these problems.

